Decentralized Search and Track with Multiple Autonomous Agents

In this paper we study the problem of cooperative searching and tracking (SAT) of multiple moving targets with a group of autonomous mobile agents that exhibit limited sensing capabilities. We assume that the actual number of targets is not known a priori and that target births/deaths can occur anywhere inside the surveillance region. For this reason efficient search strategies are required to detect and track as many targets as possible. To address the aforementioned challenges we augment the classical Probability Hypothesis Density (PHD) filter with the ability to propagate in time the search density in addition to the target density. Based on this, we develop decentralized cooperative look-ahead strategies for efficient searching and tracking of an unknown number of targets inside a bounded surveillance area. The performance of the proposed approach is demonstrated through simulation experiments.

==> systemOverview.tex <==
\section{System Overview} \label{sec:system_overview}
Before discussing in detail the proposed framework we give in this section an overview of the proposed system architecture as illustrated in Fig. \ref{fig:sysarch}. The proposed system architecture can be divided into two parts namely a) independent SAT operation and b) cooperative multi-agent SAT operation. 
An independent SAT operation occurs when an agent does not find any other agents inside its communication range. In this case the agent will optimize its individual SAT objective without cooperating with other agents. An agent commence in search mode will remain in searching until one or more targets have been detected inside its sensing range; in which case the agent will switch to tracking. An agent maintains a representation of the surveillance area which is used to indicate the areas already been searched. A particular location inside the surveillance area is marked as searched when it resides inside the agent's sensing range. That said, the agents can perform searching even when they are in tracking mode. In other words while in tracking mode, an agent can mark unvisited areas as visited and discover new targets to track. In this case however, tracking is optimized and not searching (i.e. the searching is a side effect of tracking a target over a particular area). 

To achieve the search-and-track objective, the agent maintains and propagates in time the SAT probability hypothesis density $D_k(x|Z_{1:k})$ which encapsulates the target and search density at $x$. Please note that for the rest of the paper, $D_k(x|Z_{1:k})$ will denote the proposed SAT-PHD instead of the regular PHD. The proposed predictor-corrector recursion is shown in Fig. \ref{fig:sysarch}. The predictor step produces the predicted SAT-PHD $D_{k|k-1}(x|Z_{1:k-1})$ from which the predicted search density and target density are extracted and then the search values, the target states ($\hat{X}_{k|k-1}$) and the number of targets ($\hat{n}_{k|k-1}$) are estimated. Based on these estimates, the system generates a search plan if no targets have been detected, or a track plan otherwise. In other words, the SAT controller finds the optimal control action $u_k \in \mathbb{U}_k$ for the next time step. Then, the agent moves to the new state, where it receives the measurement set $Z_k$ which is used to compute the posterior SAT-PHD (i.e. corrector step), and from which the posterior multi-target state $\hat{X}_k$ is estimated, and the search values are updated. The previous recursion is repeated over time. 

When one or more agents are in communication range they cooperate in order to solve the SAT problem more efficiently. In particular, every time that a group of agents are in communication range they exchange information (i.e. search maps) and produce a joint search plan in order to efficiently search the surveillance region (i.e. generate search trajectories that will guide the agents to search non-overlapping regions, thus maximizing the total searched area). Additionally, when one or more agents have overlapping sensing ranges they communicate in order to detect a tracking overlap i.e. a situation where two or more agents track identical targets. When this happens, the overlapping agents split and switch to search mode. 
 
